Documentation Practices in Agile Software Development: A Systematic Literature Review

Context: Agile development methodologies in the software industry have increased significantly over the past decade. Although one of the main aspects of agile software development (ASD) is less documentation, there have always been conflicting opinions about what to document in ASD. Objective: This study aims to systematically identify what to document in ASD, which documentation tools and methods are in use, and how those tools can overcome documentation challenges. Method: We performed a systematic literature review of the studies published between 2010 and June 2021 that discusses agile documentation. Then, we systematically selected a pool of 74 studies using particular inclusion and exclusion criteria. After that, we conducted a quantitative and qualitative analysis using the data extracted from these studies. Results: We found nine primary vital factors to add to agile documentation from our pool of studies. Our analysis shows that agile practitioners have primarily developed their documentation tools and methods focusing on these factors. The results suggest that the tools and techniques in agile documentation are not in sync, and they separately solve different challenges. Conclusions: Based on our results and discussion, researchers and practitioners will better understand how current agile documentation tools and practices perform. In addition, investigation of the synchronization of these tools will be helpful in future research and development.

==> sec_discussion.tex <==
\subsection{Information to document in ASD} 

We compiled a list of key information that current agile practitioners document, as well as tools and strategies for doing so. In some of the research papers that we analyzed, developers mentioned documenting key information very useful. Particularly, documentation based on the key factors helped a lot whenever there is a new team member or someone needs to catch up with the work.  

When it comes to agile software documentation, most practitioners weigh documenting user stories. Some researchers think that user stories themselves can be an alternative to documentation; however, the rest of the practitioners perceive a necessity of formal documentation of user stories. The quality requirements (non-functional requirements) are critical to document, and there are even several factors that influence documenting quality requirements in ASD \cite{9226305}. In general, documenting UI structure, architecture, API references, and test specifications is part of generic software development documentation. Agile practitioners also mentioned their inclusion in the documentation.  

Another notable fact is that current practices of agile document generation processes are based on documenting user stories, requirements, source code, architecture, and API references. Although not many practitioners mention source code to document explicitly, several workable documentation tools focus on generating source code documentation with minimal effort. 


\subsection{Roles of tools and methods}

We found a total of 23 tools and methods and classified them under ten categories based on their documentation type. The source code-based documentation category is the largest category with six tools. These tools can generate documentation from source code comments. They work as standalone or extend existing documentation tools such as Javadoc. Some of them can even attach meaningful diagrams with the source code. Wiki-based documentation type tools are effortless, and some current modern tools have evolved, inheriting the features that wiki-based tools have.

Having 23 tools and methods in 10 categories means that agile documentation tools are quite diverse based on their role. However, there is also a cost associated with it. The research papers that covered the tools are also quite disparate. They are working on several aspects, and there is a lack of combined evaluation of the existing documentation tools. 

We noticed various documentation tools based on machine learning and NLP in modern software engineering. However, in the literature, particularly on agile development, we only got one documentation tool named JavadocMiner, based on NLP. That means there are scopes for improving documentation in agile software documentation.

\subsection{Improvement of documentation workflow}

%\begin{figure}[htbp]
%\centerline{\includegraphics[width=9cm]{photos/tools-solutions-venn-di%agram.jpg}}
%\caption{Venn diagram of tools covering challenges}
%\label{figure:barcharttoolsolutionsvenndiagram}
%\end{figure}

In agile, one of the main challenges to combat is minimal documentation. We saw most of the tools presented their solution to resolve this challenge. 13 of the tools successfully provided meaningful, lean, and simple documentation. However, other tools covered challenges such as neglecting nonfunctional requirements, low-quality user stories, improper architecture, etc. 

One thing that was quite apparent was that only a couple of tools cover more than one challenge. For example, TraceMan provided solutions for three challenges, and the abstract specification tool resolved two challenges. All other tools provided solutions for only one challenge. That means these documentation tools and methods are not applicable as a complete package so that agile practitioners can use those as one place solution. 

==> sec_related_work.tex <==
In the past two decades, researchers have been studying challenges, benefits, case studies, popularity, and more on agile processes.  Kasauli et al. \cite{8049141} mentioned that information might be insufficient for developers if the team only focuses on minimizing documentation effort by documenting only user stories and test cases. Heck and Zaidman \cite{heck2017framework} proposed to omit some information (e.g., use cases, UI mock-ups) that they thought might not be mandatory at the early stage. Habib and Romli \cite{9522254} investigated many issues that might not be mandatory in agile documentation and followed a systematic mapping approach to find those out.

Over time, many researchers have formulated different tools, technologies, and approaches to improve software documentation. For example, Bayer and Muthig \cite{1607376} presented view-based software documentation and showed that the quality of documentation is directly related to its use. Moreover, Forward and Lethbridge \cite{10.1145/585058.585065} conducted a survey to uncover the perceived relevance (or lack thereof) of software documentation and the tools and technologies used to maintain, verify and validate such documents. This study also highlights the inclination for and dislikes against software documentation. Finally, Correia \cite{correia2008extending} explored the wikis that allow the collaborative creation and edition of Web page content using a web browser and showed that wikis are capable and can bring benefits when used to support different software artifacts and document types. %However, it is still not practical to support all documentation activities along the development process using the existing solutions.

There are many existing studies targeting documentation in agile software projects. Voigt et al. \cite{7521550} provided an overview of the central conceptual ideas for an agile documentation tool and conducted a survey that revealed keeping documentation up-to-date, keeping information traceable, and facilitating documentation quality assurance to be the three main requirements for documentation tools. Stettina \cite{10.1145/2038476.2038509} stated that agile practitioners do not seem to agree with the agile principle that “The most efficient and effective method of conveying information to and within a development team is face-to-face conversation.” They also found that agile teams adopt collaboration tools to share and work on agile artifacts. 
%Scrum dedicated software is perceived as essential and helpful to support the method. They figured out that instant messaging is perceived as a beneficial “backchannel” and supports documenting decisions. They have concluded that integrating software tools into the process is crucial.

%Agile documentation is one of the most talked topics in these days. B Selic in his paper \cite{5287001} suggested that documenting software at the code level is foolish; this simply results in the nightmare of trying to keep duplicated information consistent. Instead, we need design documentation at a higher level of abstraction, stripped of unnecessary technological detail and closely coupled to application concepts and requirements. He talked about agile design documentation, which keeps steps with design and development. To avoid waste, the effort expended on such documents should be proportional to the design’s stability. That is, the more stable the design, the more extensive the documentation. However, even in the earliest stages, the documentation must be adequate to serve its primary communications purpose. In a study\cite{Rubin2011}, Eran Rubin and Hillel Rubin examined the relationship between software and documentation. They developed an approach that enables incorporating domain documentation to agile development, while keeping the processes adaptive. They also provided a system design that actively uses domain knowledge documentation. These ideas have been applied through the implementation and the use of agile documentation support components.

Software developers use numerous documentation generation tools and methods as they are very convenient and effortless to generate documentation from source code comments or artifacts. McBurney and Mcmillan \cite{10.1145/2597008.2597149} proposed a technique to generate documentation via source code summarization and found that programmers benefit from their generated documentation because it includes context information. Peroni et al. \cite{peroni2013tools} conducted a similar study and proposed three tools that can be used automatically to create documentation. Spinellis \cite{5484109} explained why developers use automatic documentation generation tools. As developers are, by definition, always trying to offload tedious work to a computer, there’s no shortage of tools to handle the documentation’s drudgery. Most useful are those that create online documents by extracting text from specially formatted comments. 
%The use of Javadoc is now standard practice in the Java world. Doxygen offers similar functionality for other languages, and many C and C++ programs rely on it. Interestingly, both tools (Javadoc via the UMLGraph plug-in) can reverse engineer the code to create class diagrams. This is a case where we get valuable documentation, the proverbial picture worth a thousand words, for free.

%There are organization-wide approaches to improving software documentation, but these approaches did not provide enough evidence if those are compatible with ASD. Some papers entailed direct engagement with the documentation in agile software projects; however, they did not draw anything on how this approach will impact the time and cost of ASD. The validation of the potential use of agile documentation with ASD is also missing. In this study, we find the key practices to incorporate in agile documentation, roles of different documentation generation tools and methods, and their effectiveness in agile software development. 


%When answering research question 1, we found the key factors to add in agile documentation. Automatic document generation tools claim they have superiority and simplicity when creating the documentation. As agile depends on incremental, simple, and small steps, we anticipated the practical usability of these document generation tools in agile development. 
%However, not much validation was performed in the prior work. 
%Answering the RQ2 and RQ3, we can decide the role of agile documentation tools and methods, and how they contribute to agile software documentation.
